A New Machine Learning Dataset of Bulldog Nostril Images for Stenosis Degree Classification

Brachycephaly, a conformation trait in some dog breeds, causes BOAS, a respiratory disorder that affects the health and welfare of the dogs with various symptoms. In this paper, a new annotated dataset composed of 190 images of bulldogs' nostrils is presented. Three degrees of stenosis are approximately equally represented in the dataset: mild, moderate and severe stenosis. The dataset also comprises a small quantity of non stenotic nostril images. To the best of our knowledge, this is the first image dataset addressing this problem. Furthermore, deep learning is investigated as an alternative to automatically infer stenosis degree using nostril images. In this work, several neural networks were tested: ResNet50, MobileNetV3, DenseNet201, SwinV2 and MaxViT. For this evaluation, the problem was modeled in two different ways: first, as a three-class classification problem (mild or open, moderate, and severe); second, as a binary classification problem, with severe stenosis as target. For the multiclass classification, a maximum median f-score of 53.77\% was achieved by the MobileNetV3. For binary classification, a maximum median f-score of 72.08\% has been reached by ResNet50, indicating that the problem is challenging but possibly tractable.

==> ajustes.tex <==
\newcommand{\nomeEditor}{Binshan Lin}
\newcommand{\nomeArtigo}{A New Machine Learning Dataset of Bulldog Nostril Images for Stenosis Degree Classification}
\newcommand{\nomeRevista}{Expert Systems with Applications}
\newcommand{\nomeAutor}{Gabriel Toshio Hirokawa Higa}

